On Finite Entailment of Non-Local Queries in Description Logics

We study the problem of finite entailment of ontology-mediated queries. Going beyond local queries, we allow transitive closure over roles. We focus on ontologies formulated in the description logics ALCOI and ALCOQ, extended with transitive closure. For both logics, we show 2EXPTIME upper bounds for finite entailment of unions of conjunctive queries with transitive closure. We also provide a matching lower bound by showing that finite entailment of conjunctive queries with transitive closure in ALC is 2EXPTIME-hard.

==> ALCQ.tex <==
\subsection{\ALCQt, single role, UCQ}
As usual, we will show that existence of a counter-example is equivalent to existence of a special tree.

\subsubsection{From finite counter-example to tree} Lets start with finite interpretation \I. 
We  will proceed with a variant of a standard unravelling. We will assume that every vertex in partially constructed tree \T is labelled by a path of elements of \I. Moreover each vertex will have exactly the same concepts as the last element of its path. Two vertices are connected if path of the source is the path of the target without the last element.

Consider a vertex $v\in \T$ such that $v$ does not have all required witnesses in \T . From the path $p_v$ labelling $v$ we extract the last element $a_v\in \I$. We will construct witnesses for $v$ from witnesses for $a_v$. Let $b$ be a witness for $a_v$. It is reachable form $a_v$ by some path $p_b$ (possibly just element $b$). For every nonempty prefix $p'\preceq p_b$ we add a new vertex to the tree \T labelled by path $p_v\cdot p'$ with the same concepts as the last element in $p'$.  

The construction above obviously guarantees that all at-least requirements are satisfied. We have to check whether the at most restrictions are satisfied. Consider a vertex $v\in \T$ and let $a_v$ be the last element in the label of $v$. By construction $v$ has the same concepts as $a_v$ and successors of $v$ map injectivelly into successors of $a_v$. Therefore any at-most restriction for $v$ cannot be violated, since any such restriction was not violated for $a_v$.


There is a natural homomorphism from \T into \I , so no query not satisfied it \I can be satisfied in \T .    


\subsubsection{From trees to finite couter-exaples}

Folding tree into finite structure will be a bit more complicated than in the case \ALCIt due to long at-least restrictions. 
For each concept $A$ we will introduce finite number of {\em shades} such that
\begin{itemize}
 \item every vertex with concept $A$ will get exactly one shade of $A$ as a new concept
 \item if a vertex has a restriction $\geq ^nr^+.A$ then among its descendants there are $n$ different shades of $A$
\end{itemize}
This will be done inductively in a greedy fashion. We will keep the following invariant: In the tree rooted in an unprocessed vertex each shade of each concept $A$ is used at most once. In a tree without any concept shades the invariant is trivially satisfied.

Take a n unprocessed vertex $v$ closest to the root. Suppose $v$ has a restriction of the form $\geq ^nr^+.A$. If at least $n$ of its descendants have assigned shades of $A$, then we proceed. Otherwise use some unused shades to color descendants of $v$. Notice, that we will never have to use more shades that the highest number used in the T-box.


For each concept (including shades) $C$ add a new concept $C_{\exists r\trans. C}$  axiomatizated by two inclusions: $C_{\exists r\trans. C} \sqsubseteq \exists r\trans. C$ and $\overline{C_{\exists r\trans. C}} \sqsubseteq \forall r\trans. \bar C$. Finally, we add colours  for coloured blocking principle.

Now consider a level $l$ in this tree such that all neighborings large enough for coloured blocking principle   realized in the model are present above this level.
For all nodes above level $l$ and each applicable concept choose any witness.
Preserve this witnesses and paths to them; fold the rest of the tree, redirecting the edges above level $l$.

The only nontrivial thing to check at this point is whether long at-least restrictions are satisfied. But that follows from the observations that each element satisfies its long existential restrictions for shades of concepts. 


\subsubsection{Complexity}
Existence of appropriate tree will be checked by automaton. The information needed for automaton contains:
\begin{itemize}
 \item unary type of a vertex
 \item for each $A\in CN(\K)$, the minimum number of elements with concept $A$ in a given subtree
 \item for each $A\in CN(\K)$, an indicator whether we made progress looking for  
elements in concept $A$.
 \end{itemize}

All together the size of automaton is equal to $(2\cdot 2 \cdot t)^{|CN(\K)|}$. As usual, we take the product of above automaton with automaton recognizing the query.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> UCQplusconceptqueries.tex <==

\subsubsection{Concepts for the query}
Assume that there are no inverse roles in the atoms of $Q$; that is, replace each $r^-(x, y)$ with $r(y, x)$ and each $(r^-)\refltrans(x, y)$ with $r\refltrans(y, x)$.\nb{In this section I use reflexive transitive closure.}

Consider an \ALCOIt-tree.
The idea is to enrich the interpretation with concepts $C_{P, W}$ for $P$ being a \CQt from some class of queries and $W$ being a nonempty subset of $\var(P)$.
Such a concept will be present in all elements $x$ for which there exists a match for $P$ such that all variables from $W$ are mapped to $x$ and the whole match is contained in the subtree of $\Bag(x)$ (that is, all variables are mapped to elements in this subtree and all witnessing paths are in this subtree).
Then we will also introduce a concept $C_P$ present in the elements in which any $C_{P, W}$ is true.

We want to do it in a way possible to verify by the procedure above: that is, the new concepts will be axiomatized by concept inclusions and by forbidding some patterns in a bag (by a \UCQt).

\begin{definition}
We say that a \CQt $Q$ is \emph{connected} if for any two variables $x, y \in \var(Q)$ there is a sequence of variables $a_1, a_2, \dots, a_n$ such that $a_1 = x$, $a_n = y$ and for each pair of subsequent variables $a_i, a_{i+1}$ there is a role name $r$ such that one of the following atoms is in $Q$: $r(a_i, a_{i+1})$, $r(a_{i+1}, a_i)$, $r\refltrans(a_i, a_{i+1})$ or $r\refltrans(a_{i+1}, a_i)$.
\end{definition}

Reduce the entailment problem for arbitrary \UCQt to the problem for a single, connected \CQt.
Assume that $Q$ is a \UCQt and $Q = Q_1 \lor Q_2 \lor \dots \lor Q_n$, where each $Q_i$ is a \CQt.
First, we will show that we can assume that each $Q_i$ is connected.
Take any $Q_i$ and let $P_1, P_2, \dots, P_m$ be its connected components.
Choose one connected component for each $Q_i$ and ask for the query entailment of the disjunction of the chosen connected components; if for any choice of connected components the query is not entailed, then the whole query $Q$ is not entailed (with the same counter-model).
On the other hand, if $Q$ is not entailed, there exists a counter-model, and there is a choice of the connected components of each $Q_i$ which do not have a match in this counter-model.

Now, the reduction from a disjunction of connected queries to a single \CQt: assume we have already defined concepts $C_{Q_i}$ for each $Q_i$.
We can forbid some patterns inside a bag.
Thus, we can forbid a CQ $C_{Q_i}(x) \land \overline{C_Q}(x)$ for each $Q_i$ (and a fresh variable $x$) in every bag, thus assuring that if any element of the interpretation has concept $C_{Q_i}$ for any $i$, it also has concept $C_Q$.

Now we can assume that $Q$ is a single, connected \CQt.
We will define a class $C$ of queries (\CQt) for which the above concepts will be defined.

The description of the class $C$ is quite simple: first, replace each transitive atom $r\refltrans(x, y)$ in $Q$ with $r\refltrans(x, z) \land r\refltrans(z, y)$ for a fresh variable $z$ (we distinguish one node on each witnessing path; the intended meaning is that the distinguished node is some element of the highest bag through which the witnessing path passes).
We will call each such variable $z$ a \emph{distinguished variable}.
Note that each transitive atom has exactly one endpoint being a distinguished variable.
The class $C$ consists of all subqueries of $Q$ (including itself).

Now we want to axiomatize concepts for a query $P \in C$ and $W \subseteq \var(P)$.
Recall that the concept $C_{P, W}$ is supposed to be satisfied in an element $x$ if that there is a match of $P$ contained in the subtree of $\Bag(x)$, mapping all variables from $W$ to $x$.
We will define the axiomatization and prove this implication at the same time.

The left column of the table below corresponds to the proof, and the right one to the axiomatization of $C_{P, W}$.

We will look at a match for the query as a graph consisting of all witnessing paths and edges required by the query.

\begin{center}
\begin{tabular}{ m{2in} | m{1.3in} }
Assume there is a match $M$ for $P$.
Let $v$ be the highest (closest to the root) bag with nonempty intersection with the match.
Note that any witnessing path has the image of a distinguished variable as one of its endpoints.
For all witnessing paths passing through $v$, if the distinguished endpoint is not mapped to an element of $v$, let us remap it to some element of $v$ on the path (as each distinguished variable occurs only in two atoms, it is easy to see that the match is still correct).
Let $V$ be the set of elements of $v$ to which any variable is mapped. & Consider all possible subsets of variables $V' \subseteq \var(P)$. \\
\hline
For any witnessing path with one endpoint inside $V$ and the other outside $V$ (thus, outside of the bag $v$), mark the last element of $v$ on this path (that is, for a witnessing path beginning in $x \in V$, consider its longest prefix that is contained in the bag $v$ and mark the last element of this prefix).
Add all marked elements to $V$. &
For any transitive atom $r\trans(x, y)$ with one endpoint inside $V'$ and the other outside, take a fresh variable $z$ and replace the atom with $r\trans(x, z) \land r\trans(z, y)$.
Add $z$ to $V'$. \\
\hline
 & Guess which variables are mapped to the same element (i.e. consider all possible contractions; we will discard some of them).
 Let $R$ be such a ``contracted'' query.\\
\hline
Let $M_{in}$ be the match $M$ restricted to $V$ (viewed as graphs, $M_{in}$ is the subgraph induced by $V$).
Note that $M_{in}$ is connected.
Let $M_{out}$ be $M$ without the edges from $M_{in}$. &
Consider $R$ restricted to $V'$ (call it $R_{in}$) and the rest of the query $R_{out}$.
If $R_{in}$ is not connected, discard the query $R$. \comment{(maybe we don't need this?)} \\
\hline
Let $M_x$ denote a connected component of $x$ in $M_{out}$.
Consider any two different elements $x, y \in V$.
Note that $M_x$ and $M_y$ are disjoint (their elements, apart from $x$ and $y$, are in different subtrees and there are no witnessing paths between them, as they would pass through $v$, and we made sure that all such paths are split by the distinguished variables). &
For each variable $x \in V'$, let $R_x$ be the query $R_{out}$ restricted to the connected component of $x$.
If for any distinct $x, y \in V'$, $R_x$ and $R_y$ are not disjoint, discard the query R. \\
\hline
Now consider $M'_x$ as $M_x$ with $x$ removed.
$M'_x$ might consist of several connected components.
Each component is contained in the subtree of some child of $v$, connected directly to $x$.
Thus, all witnessing paths from $x$ to this connected component must pass through the entrance node of this child. &
Let $R'_x$ be $R_x$ with $x$ (and all atoms involving it) removed.
$R'_x$ might consist of several connected components.
Let $X$ be one such component.
All atoms in $R_x$ involving $x$ and one of the variables from $X$ must concern the same role; if this is not the case, discard $R$.
\end{tabular}
\end{center}
It should be clear that each match $M$ has a corresponding ``contracted'' query $R$ which captures the structure of $M$ in the bag $v$.
For each query $R$ that was not discarded, we will create auxiliary concepts $C_{R,x}$ for $x \in \var(R)$, intended to capture the corresponding matches $M$.
Now we will describe these concepts.

Recall that $R = R_{in} \land R_{out}$, as described above.
The match for the part $R_{in}$ has to be contained inside one bag.
As for $R_{out}$, for each variable $x$ from $\var(R)$, consider each connected component $X$ of $R'_x$.
Let $N(x)$ be the set of all variables $y \in \var(X)$ such that there is a non-transitive role atom in $R_x$ involving $x$ and $y$.
Furthermore, for each transitive atom involving $x$ and a variable from $X$, let $z$ be the distinguished variable corresponding to that atom \todo{describe the correspondence; the atom was probably created by splitting some transitive atom from $P$, and it had a distinguished variable as one endpoint} (think of $z$ as a fresh variable); add this atom to $X$, but with $z$ instead of $x$.
Let $D(x)$ be the set of all such distinguished variables.
Then the query for the connected component $X$ is $C_{X, N(x) \cup D(x)}$ (and it is intended to be present in the entrance node of the appropriate child bag of $v$).
It is easy to see that $X$ constructed this way is in the class $C$.
\comment{The distinguished variables magic probably requires some comment; we do it just to assure that the resulting query is in our class (we could introduce a fresh variable for the entrance node and then show that the resulting query is isomorphic to some query from the class, but it is exactly the query above).}

Thus, to deal with $R_{out}$ we just need to assure that if an element is connected to children bags with appropriate $C_{X, N(x) \cup D(x)}$ concepts in the entrance node, it has a concept denoting it.
This can be done by introducing some auxiliary concepts and simple universal CIs speaking about the complementary concepts (or just hardcoded into the local correctness conditions in the procedure above, specifically into legal children types).
This allows us to rewrite $R$ as $R_{in}$ with some additional concept atoms.
To deal with the whole query $R$, for each $x \in \var(R)$, we forbid the pattern $R \land \overline{C_{R, x}}(x)$ (note that this is an auxiliary concept, used only inside one bag; it does not need to belong to the class $C$; we also do not consider sets of variables mapped to $x$, as in $R$ the variables are already contracted).

Finally, if $R_1, R_2, \dots, R_k$ are the contracted queries which were not discarded, the target concept $C_{P, W}$ is a disjunction of all $C_{R_i, x}$ such that the variable $x$ in $R_i$ was constructed by gluing the set $W$, possibly along with some fresh variables not present in $R$.
And, again, this disjuntion is realized as a forbidden pattern: $C_{R_i, x}(y) \land \overline{C_{P, W}}(y)$ for a fresh variable $y$.

We need to also show that if there is any counter-model, there exists its conservative extension with an empty interpretation of $C_Q$.
This is straightforward: just let $C_{P, W}$ be true in an element $x$ iff there is a match of $P$ with all variables from $W$ being matched to $x$ (and $C_P$ be true if any of $C_{P, W}$ is true).
As it was a counter-model, $C_Q$ will not be satisfied, and if some part of axiomatization of $C_{P, W}$ is violated in some element $x$ (i.e. some of the forbidden patterns are violated -- note that without them all concepts $C_{P, W}$ might as well be interpreted as the whole domain), it is straightforward to construct a match for $P$ with all variables from $W$ being matched to $x$.


==> UCQplusfold.tex <==
\subsection{Folding back the model}
\begin{definition}
An interpretation is \emph{$\ell$-bounded} if each simple directed path has length at most $\ell$.
\end{definition}
Having the concept $C_Q$, we can add to all considered KBs a CI $C_Q \sqsubseteq \bot$.
Then the procedure decides whether there exists a strong counter-example.
If it exists, there is a regular witness $(\Imc, T)$ with $T$ having bounded degree $d$ and a bound $m$ on the length of a simple directed path.
Because the tree $T$ is regular, $\Imc$ also has bounded degree and is $\ell$-bounded for some $\ell$ (there are finitely many non-isomorphic subinterpretations in the tree partition $T$ and all of them are finite).
Assume that $\Imc$ is infinite (otherwise there is no need to fold back).
Let $Q\refltrans$ be obtained from $Q$ by replacing each transitive atom $r\refltrans(x, y)$ with a disjunction:
\[ \bigvee_{i\leq \ell} r^i(x, y), \]
where $r^i(x, y)$ expresses existence of an $r$-path of length $i$ from $x$ to $y$ (i.e. for $i=0$ it states that $x = y$; for $i = 1$ it is $r(x, y)$, and for $i > 1$ it is $r(x, z_1) \land r(z_1, z_2) \land \dots \land r(z_{i-1}, y)$ for fresh variables $z_1, \dots, z_{i-1}$). Rewrite $Q\refltrans$ as a UCQ (in the disjunct for $i = 0$, all occurences of the variable $y$ are replaced with $x$). Let $k$ be a bound on the number of binary atoms in one CQ in $Q\refltrans$.

\begin{lemma}
For all $\ell$-bounded interpretations $\Jmc$, $\Jmc \models Q$ iff $\Jmc \models Q\refltrans$.
\end{lemma}

For any $n$, let $\Imc_n$ be any $n$-proper colouring of $\Imc$. \todo{write the definition of $n$-proper colourings}
Fix $n = \max(\ell^2, k^2)$. \todo{verify the bounds}
On each infinite branch $\pi$ of $T$, consider the set of nodes (bags) $V_\pi$ on $\pi$ such that $v \in V_\pi$ if the role of $v$ if $r$, but the role of its parent is $r^-$ (there are infinitely many such bags, because lengths of simple directed paths in $T$ are bounded and $\pi$ is infinite).
Let $D_\pi \in V_\pi$ be the first node for which there exists an earlier node $E_\pi \in V_\pi$ such that $N^{\Ii_n}_n(d_\pi)\simeq N^{\Ii_n}_n(e_\pi)$, where $d_\pi \in D_\pi$ and $e_\pi\in E_\pi$ are entrance nodes.
An interpretation $\Ff_n$ is obtained by including the branch $\pi$ up to the predecessor of $D_\pi$ and the edge originally leading to $d_\pi$ is redirected to $e_\pi$.

\begin{lemma}
After any number of redirections, there are no paths of lengths greater than $\ell$.
\end{lemma}
\begin{proof}
There can be no directed path passing through more than one redirected edge -- each edge is redirected to a bag over role $r$, and at all times all edges leaving this bag are by $r^-$.
For a single redirect, for any path passing through the redirected edge, a corresponding path of the same length can be easily found in the model before the redirection.
\end{proof}

\begin{lemma}
$\Ff_n \models \Kk$.
\end{lemma}
\begin{proof}
We need to be sure that there is no $r$-path from $e_\pi$ to $d_\pi$ (otherwise the KB could be violated, as $e_\pi$ might require some witness below $d_\pi$).
This is guaranteed by taking neighbourhoods of size larger than $l$ (bound on the length of a simple directed path).
\end{proof}


By the coloured blocking principle, $\Ff_n \not\models Q\refltrans$, and as it is $\ell$-bounded, $\Ff_n \not\models Q$.
Thus, there exists a finite counter-model.


==> UCQplusprocedure.tex <==

\subsection{Finding a strong counter-example}
First we will assume some additional properties of the strong counter-example that we will look for.
\begin{lemma}
If there is any strong counter-example, there is also one with the following property: for every element $x$, in the subtree of $\Bag(x)$ there are all witnesses required for $x$ by existential CIs in the TBox of $\Kk$.
\end{lemma}
\begin{proof}
(sketch) For any element $x$ we can duplicate the subtree of $\Bag(x)$ (there is an obvious homomorphism, so nothing changes wrt. KB and query).
We can also root the tree in another bag, duplicate some subtree and restore the original root.
Thus, if the required witnesses are not in the subtree, we can just duplicate whole interpretation apart from the subtree and add the copy as a fresh child.
\end{proof}

\begin{definition}
A \emph{bag type} of a non-root bag $v$ of an SCC-partition is the following triple:
\begin{itemize}
  \item the role $r_v$ on the label of the incoming edge in the tree (this is either $r$ or $r^-$, where $r$ is the unique role used by $\Kk$);
  \item the unary type $\tau_v$ of its entrance node $e_v$;
  \item the set $\Reach$ of concept names reachable from $e_v$ by $r_v$ (in the subtree of $v$ -- this is implicit, because the only edge pointing upwards the tree is by role $r_v^-$).
\end{itemize}
\end{definition}
\begin{lemma}
If there is any strong counter-example $(\Imc, T)$, there is also one with the following property: for any element $x \in \Delta^\Imc$, bag types of children of $\Bag(x)$ such that there is an edge from $x$ to the entrance node of this bag are distinct. \todo{state it more clearly}
\end{lemma}
\begin{proof}
If there are two children of $\Bag(x)$ with the same bag type and with edges from $x$ to the entrance nodes of both of them, one of these edges (and one of the children, along with its whole subtree) can be removed.
Removing some elements cannot make the query satisfied; and as the bag type contains information about the unary type of the entrance node and all concepts reachable from it by the role of the incoming edge, all the witnesses required by CIs in subtree of one of the children can be found also in the subtree of the other one.
\end{proof}

Consider some strong counter-example $(\Imc, T)$ and any bag $v$ from $T$.
One can look at the subtree rooted in $v$ (and the corresponding subinterpretation of $\Imc$, along with the nominals) as a strong counter-example for the same query and different KB, with ABox containing only one individual with fully specified unary type (corresponding to the entrance node of $v$) and the same TBox as $\Kk$.
% For $v$ of bag type $\tau$, we will call it an \emph{\ALCOIt-tree for bag type $\tau$}.
The intermediate goal is to develop a procedure calculating the set of bag types for which such a strong counter-example exists.
At the end we want to reduce this problem to the existence of an interpretation corresponding to a single bag, assuring some simple local conditions between the bag and its children.

We will describe the procedure determining existence of a strong counter-example by describing simpler procedures and gradually getting nearer the goal.
Begin with assuming that the query is trivial; thus, we want to find any safe model of $\Kk$.
The strategy is to search for an appropriate \ALCOIt-tree (we will still call it a strong counter-example, even though the query is trivial).

Let $\tau = (r, \sigma, R)$\vic{THis notation needs to be introduced} be a bag type and $T$ be a set of bag types.
The situation we consider is a bag of type $\tau$ with children of types from the set $T$ (the types of children can repeat and not all types from $T$ has to be used).
We want to define some \emph{local correctness conditions} that must be satisfied in such a situation (essentially: existence of a model of a single bag; but as some witnesses required by the TBox might be present in the subtrees of its children, it depends on the bag types of children).
Namely, we will construct an \ALCOIt-knowledge base $\Kk_{\tau, T}$ and a non-transitive UCQ $Q_\tau$ such that if $\Kk_{\tau, T} \fentails Q_\tau$, there is no strong counter-example in which the considered situation occurs (i.e. there is a bag of type $\tau$ with children of types from $T$).

We will first construct an auxiliary knowledge base $\Kk_\tau$, independent of $T$.
Begin with the copy of the TBox of $\Kk$ restricted to the role $r$.
For every concept $B$ add fresh concepts $B_{in}, B_{out}, B_{exit}, B_{any}$ and the following CIs:
\begin{itemize}
  \item $B_{in} \sqsubseteq \exists r\trans. B$,
  \item $B_{out} \sqsubseteq \exists r\trans. B_{exit}$,
  \item $B_{any} \sqsubseteq B_{in} \sqcup B_{out} \sqcup B_{exit}$,
\end{itemize}
and replace every CI of the form $A \sqsubseteq \exists r\trans. B$ by a CI $A \sqsubseteq B_{any}$.
The concepts $B_{in}$ are supposed to be satisfied in the elements that can reach concept $B$ inside the bag;
$B_{exit}$ -- in the elements from which there exists an $r$-edge going to some child bag with reachable concept $B$;
$B_{out}$ -- the ones that can reach $B$ outside the bag through $B_{exit}$;
$B_{any}$ -- any of the above.
Finally, set the ABox of $\Kk_\tau$ to $\{A(b) \mid A \in \sigma\} \cup \{A_{any}(b) \mid A \in R \}$ (recall that $R$ is the third component of the bag type $\tau$ -- the set of concepts reachable from the entrance node by $r$).

Now construct $\Kk_{\tau, T}$.
Begin with a copy of the ABox and all non-existential CIs of $\Kk_\tau$.
We need to know which existential CIs need to be satisfied inside the bag, and which ones will have witnesses in the children (or their subtrees).
To deal with this, we will assume that each element $x$ of the resulting model has edges to all possible bag types from $T$, as long as this does not invalidate the knowledge base.
Checking whether adding an edge to the model invalidates the knowledge base requires just looking at the unary types of its endpoints.
As a result, for each unary type $\sigma$ in $\Kk_\tau$ we can easily calculate the set of its \emph{legal children types}: the bag types for which the edge from an element with unary type $\sigma$ to the entrance node of such a bag type does not invalidate the knowledge base.
Add to $\Kk_{\tau, T}$ a fresh concept $A_\sigma$ for each unary type $\sigma$ in $\Kk_\tau$, with the natural axiomatization.
For each such unary type $\sigma$ and each existential CI $C$ of the form $A \sqsubseteq \exists r. B$ from $\Kk_{\tau}$ (where $A \in \sigma$), check whether $C$ is witnessed in any of its legal children types (i.e. if the unary type of its entrance node contains $B$).
If not, add to $\Kk_{\tau, T}$ a new CI $A_\sigma \sqsubseteq \exists r. B$.
Similarly add all transitive existential CIs not witnessed in the legal children types (i.e. if no legal children bag type has an appropriate concept in the set $\Reach$ of reachable concepts).
Additionally, there are two cases in which the unary type $\sigma$ becomes forbidden.
If $\sigma$ contains a concept $B_{exit}$ for some $B$, check whether any of its legal children types by role $r$ has $B$ in the set of reachable nodes; if not, this unary type is forbidden.
Also, for the existential CIs involving roles other than $r$, if there is at least one of them which is not witnessed by the legal children types, $\sigma$ is forbidden.
Forbidding a type means that we add to $Q_\tau$ a simple CQ $\bigwedge_{A \in \sigma} A(x)$ for a fresh variable $x$.\nb{This can be either in the query or we can use the finite entailment modulo types; I'm not sure how it influences the complexity.}

\subsubsection{The procedure}\vic{What are the realizability/compatibility conditions to decide when to eliminate a type}
The algorithm will be a variant of type elimination \cite{Pratt79,abs-1202-0914}.\CHECK
Begin with the set of all possible bag types $T_0 = \Rol(\Kk) \times \Tp(\Kk) \times \Pp(\Tp(\Kk))$.
For $T \subseteq T_0$ let $F(T)$ be the set of types $\tau \in T$ such that there exists a finite model of $\Kk_{\tau, T}$.
Note that $F$ is a monotone operator on subsets of $T_0$.
Consequently, $F$ has the greatest fixed point and it can be obtained by iterating $F$ on $T_0$:
\[T_0 \supseteq F(T_0) \supseteq F^2(T_0) \supseteq \dots \supseteq F^i (T_0) = F^{i+1} (T_0) \] for some $i\leq |T_0|$.
Let $T = F^{i}(T_0)$.
Removal of some bag type $\tau$ during this procedure witnesses that if an \ALCOIt-tree contains a bag $v$ of such type, if we consider the subtree of $v$ as an \ALCOIt-tree of bag type $\tau$, it has to violate some local correctness conditions and therefore the whole \ALCOIt-tree cannot model $\Kk$.
Now we want to check whether there exists an interpretation corresponding to the root bag, realizing the ABox of $\Kk$ with children bag types from $T$.
For this, simply check the local conditions as in the case of $\Kk_{\tau, T}$, but this time copy the ABox from $\Kk$.

If the above procedure is successful, there is an \ALCOIt-tree with root bag realizing the ABox of $\Kk$.
However, it might not be safe, and therefore might not even model $\Kk$ (the transitive existential CIs might not be satisfied -- each bag type on some infinite path may have some concept in its set of reachable concepts, but it might never be actually reached).

Assuring safety requires the following modification of the above procedure.
Instead of adding each bag separately, we will add whole (finite) connected components by one role at once and assure that we add such components for alternating roles.
By a connected component by role $r$ we mean all bags reachable by role $r$ (\emph{not} by role $r^-$) from a given bag $v$, where the role of $v$ is $r$ and the role of parent of $v$ is different than $r$.

Once again, we are interested in local correctness conditions for such a connected component.
More precisely, now we are given a role $r$ and a set of bag types $S$ by roles different than $r$ (possibly $r^-$) and we consider a finite connected component of bags by role $r$ such that all edges leaving this component lead to bags of types from $S$.
This component, of course, is a tree.
We want to first calculate the set of bag types that could be the leaves of such a tree (without violating the local correctness conditions), and then, inductively, other realizable bags.
Begin with an empty set of bag types $T_0 = \emptyset$ -- allowed types of children by role $r$.
For 
\[ T \subseteq \{r\} \times \Tp(\Kk) \times \Pp(\Tp(\Kk)) \]
and
\[ S \subseteq (\Rol(\Kk)\setminus\{r\}) \times \Tp(\Kk) \times \Pp(\Tp(\Kk)) \]
let $F_S(T)$ be the set of bag types $\tau \in T$ such that there exists a finite model of $\Kk_{\tau, T\cup S}$.
As $F$ is a monotone operator on sets of bag types with role $r$, it has the lowest fixed point and it can be obtained by iterating $F_S$ on an empty set.

The whole procedure for deciding existence of a strong counter-example (for a trivial query) works as follows.
Begin with the set $T_0$ of all bag types.
Let $T[r]$ denote the set of all elements of $T$ (bag types) with the first coordinate (role) equal to $r$.
Let $F_r(T)$ be the set of types $\tau \in T[r]$ realizable by a finite connected component by role $r$ in $\Kk_{\tau, T \setminus T[r]}$.
Take any order of the roles and apply each $F_r$ to the set under construction $T$.
Repeat this procedure until $T$ stabilizes (it must happen, as each $F_r$ is monotone).
Take the resulting set of types $T$ and check, as before, whether the root bag realizing ABox of $\Kk$ has a model satisfying the local correctness conditions with children bag types from $T$.
% If it can be realized, there exists a strong counter-example for $\Kk$ and a trivial query.

\subsubsection{Correctness and regularity}
It is easy to see that, if there exists any strong counter-example, its tree of bag types is a witness that the procedure will be successful.
Assuming the contrary, if $S$ is the set of all bag types occuring in this tree, consider the first moment when any $\tau \in S$ would be removed from the set $T$ of the types considered by the procedure.
It must mean that for some set $T \supseteq S$, the type $\tau$ is not realizable by any finite connected component by role $r$ in $\Kk_{\tau, T \setminus T[r]}$, where $r$ is the role of $\tau$.
However, $\tau$ is a part of some finite connected component in the strong counter-example.
By considering all bag types in this connected component, bottom-up, one can easily check that the procedure will not remove $\tau$ from the set of considered bag types.

For the other direction: if the above procedure is successful, it essentially calculates a regular infinite tree of bag types, such that there exists an interpretation for each of these bags which is locally correct.
For each bag type $\tau$ and each set of bag types $T$ such that in this tree there is a bag type $\tau$ with children of types $T$, fix some model $\Imc_{\tau, T}$ of $\Kk_{\tau, T}$.
Fix also any model of the KB for the root bag. \todo{Define it earlier properly and name it somehow?}
Let $\Imc$ be the interpretation consisting of all chosen interpretations for single bags (with all instances of nominals merged), along with the edges between elements of parent bags and entrance nodes of their children (according to the assumptions inside the procedure: if an edge from $x$ to some bag type does not invalidate the knowledge base, add an edge from $x$ to one of the children with this bag type).
$\Imc$ is a model of $\Kk$: all universal CIs are satisfied inside the bags and, by the construction of the edges between the bags, cannot be violated by them.
The existential CIs are either satisfied inside bags, or are guaranteed to be satisfied in a subtree of one of the children; for the transitive ones it can be proved by a simple induction in one connected component.

\subsubsection{Bounded degree}
There are finitely many interpretations $\Imc_{\tau, T}$ of single bags that we used to construct $\Imc$.
If $k$ is the size of the biggest of them and $l$ is the number of possible bag types, the degree of the tree is bounded by $kl$ (and $l \leq |\Kk|\cdot 2^{|\Kk|} \cdot 2^{|\Kk|}$).

\subsubsection{Non-trivial queries}
For non-trivial queries only some details of the procedure change.
We will extend the knowledge base with some concepts related to the query; in particular, we will add a concept $C_Q$ such that, if there is any match for concept $Q$, the interpretation of $C_Q$ will not be empty.
To assure this, apart from the standard CIs, we will need to forbid some patterns inside the bags.
This will be handled by adding these patterns to all the queries $Q_\tau$ used when verifying local correctness conditions for a single bag and its children bag types.


==> nominals_body.tex <==
\newpage

\section{Eliminating nominals and complex ABoxes [draft]}~\label{sec:ABoxesNomMain}
Finite entailment of a \UCQt $Q$ by an $\ALCOIt$ (resp. $\ALCOQt$) KB $\Kk$ can be reduced to multiple instances of the problem of finite entailment of a $\UCQt$ by an $\ALCIt$ (resp. $\ALCQt$) KB.
Moreover, in these instances, the knowledge base can be assumed to have a trivial ABox (i.e. consisting of one individual with fully specified unary type).
The reduction does not introduce new role names\nb{right now not true for \ALCOIt; should be easy to change, but also: we don't need it for \ALCOIt}.

As we use this result several times \comment{(twice? thrice?)} and depend on the detailed complexity bounds, we state it as an algorithmic result for several different cases, providing for each of them:
\begin{itemize}
 \item the number of instances to which we reduce;
 \item three bounds on the sizes of these instances:
 \begin{itemize}
   \item size of the KB;
   \item number of disjuncts in the query (call it \emph{query length}(?));
   \item size of the largest disjunct in the query \comment{(number of atoms? variables? binary atoms?)} (call it \emph{query width}(?)).
 \end{itemize}
\end{itemize}

Let $\Kk$ be an \ALCOIt or \ALCOQt KB and $Q$ be a \UCQt with $n$ disjuncts, each of size at most $m$.

\begin{itemize}
 \item If $\Kk$ is an \ALCOIt KB, there is an exponential (in $|\Kk|$) number of instances, with size of the KB polynomial in $|\Kk|$, query length $O(|\Kk|^n)$ and query width at most $3m$.
 \item If $\Kk$ is an \ALCOQt KB, there is a double exponential (in $|\Kk|$) number of instances, with size of the KB exponential in $|\Kk|$, query length $O(2^{n|\Kk|})$ and query width at most $3m$. \todo{verify}
 \item If $\Kk$ is an \ALCOQt KB without long at-most restrictions and all but one nominal having guaranteed no outgoing edges, there is an exponential (in $|\Kk|$) number of instances, with size of the KB polynomial in $|\Kk|$, query length $O(|\Kk|^n)$ and query width at most $3m$. \todo{verify, specify the conditions}
\end{itemize}

For the full proof, see Appendix.
The main ideas of the reduction for \ALCOIt:
\begin{itemize}
 \item axiomatization of concepts $C_{\exists r. A} \equiv \exists r. A$ and $C_{\exists r\refltrans. A} \equiv \exists r\refltrans. A$ for all concepts $A$ from the original KB;
 \item after fixing the unary types of the nominals, the query can be modified to not use nominals; thus, it stays mostly the same in the instances; 
 \item we want to create a set of KBs $\Kk_i$; each KB corresponds essentially to a guess of the properties of the nominals and their neighbourhoods \comment{(court?)} (unary types, connections between them);
 \item for each model of $\Kk$, there is a model of some $\Kk_i$ being the same, but with the nominals removed (and enriched with some concept names).
\end{itemize}
For \ALCOQt similarly, but handling the number restrictions along the way; the crucial observation is that there is a bounded number of relevant successors of the nominals; thus, we can treat them all as nominals too; to get good complexity and a trivial ABox, we need one-step unravelling of the nominals.


==> transitive_atoms-inverses.tex <==
\section{Eliminating transtive atoms: \ALCIt}
Let $\Kk$ be an \ALCIt KB using only one role, let $Q$ be a \UCQt and let $T$ be a set of forbidden unary types.
We will remove the transitive atoms from the query.

We assume there just one individual.

\subsection{Tree-like structure}
We will be interested in arbitrary models and their tree partitions with the following properties:
\begin{itemize}
 \item each bag is finite;
 \item each (directed) edge between bags has exactly one associated edge in the interpretation;
 \item each edge in the interpretation is either inside one bag or is associated to some edge between bags and connects an element from the parent bag and an element from the child bag (preserving the direction of the edge between the bags);
 \item the root bag contains the individual.
\end{itemize}
We will call it an SCC-partition (as each strongly connected component needs to be inside one bag).
For each element $x$ of the interpretation define $\Bag(x)$ as the bag in the SCC-partition containing $x$.

\begin{definition}
An interpretation is \emph{safe} if it does not contain an infinite simple directed path.
\end{definition}

We will call a model $\Imc$ along with its SCC-partition a \emph{strong counter-example} if:
\begin{itemize}
 \item $\Imc \models \Kk$;
 \item $\Imc$ is safe;
 \item $\Imc \not\models Q'$, where $Q'$ is $Q$ with each transitive atom $r\trans(x, y)$ replaced with:
 \[ \bigvee_{x'\in\Bag(x)} \bigvee_{y'\in\Bag(y)} r\trans(x', y'). \]
\end{itemize}

\begin{lemma}
There exists a finite counter-model iff there exists a strong counter-example.
\end{lemma}
For the left-to-right implication we will construct a strong counter-example from any finite counter-model by unravelling it appropriately.
For the right-to-left one we will develop a procedure deciding whether there exists a strong counter-example; it will follow that if there is one, there is also one with bounded degree of its SCC-partition and it can be folded back to a finite counter-model.

\subsection{Unravelling}
Let $\Imc$ be a finite counter-model.
We will construct a finite counter-model $\Jmc$ with an SCC-partition (forming a strong counter-example).
There will be a homomorphism $h: \Delta^\Jmc \to \Delta^\Imc$, as each element of $\Jmc$ will be constructed as a copy of some element from $\Imc$.

The root bag contains the ABox along with strongly connected components of the individuals.
Then, for each element $x' \in \Delta^\Jmc$, let $x = h(x')$ (i.e. $x'$ was constructed as a copy of $x$) and consider all edges incident to $x$ in $\Imc$.
If any such edge $(x, y)$ or $(y, x)$ was not yet copied to $\Jmc$ (i.e. there is no copy $y'$ of $y$ such that there is an edge between $x'$ and $y'$), create a fresh copy of $y$ and its strongly connected component in $\Jmc$ and add an edge from $x$ to $y'$ (or an inverse one), where $y'$ is the copy of $y$.
Repeat the above for each element added to $\Jmc$.

Now each bag consists of a single strongly connected component (a copy of an SCC from $\Imc$).
No two adjacent bags can be copies of the same SCC from $\Imc$.
It is easy to verify that $\Kk$ is satisfied.

$Q$ does not have a match in $\Jmc$, because of the homomorphism $h$.

$\Jmc$ with the declared SCC-partition is a strong counter-example; each bag is an SCC, so the query $Q'$ from the definition of a strong counter-example is equivalent to $Q$; and $\Jmc$ is safe, because any two adjacent bags are copies of different SCCs, so the longest directed path in this tree is bounded by the size of $\Imc$.

\input{sections/UCQplusprocedure}
\input{sections/UCQplusconceptqueries}
\input{sections/UCQplusfold}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

